Modality-Agnostic Variational Compression of Implicit Neural Representations

We introduce a modality-agnostic neural compression algorithm based on a functional view of data and parameterised as an Implicit Neural Representation (INR). Bridging the gap between latent coding and sparsity, we obtain compact latent representations non-linearly mapped to a soft gating mechanism. This allows the specialisation of a shared INR network to each data item through subnetwork selection. After obtaining a dataset of such latent representations, we directly optimise the rate/distortion trade-off in a modality-agnostic space using neural compression. Variational Compression of Implicit Neural Representations (VC-INR) shows improved performance given the same representational capacity pre quantisation while also outperforming previous quantisation schemes used for other INR techniques. Our experiments demonstrate strong results over a large set of diverse modalities using the same algorithm without any modality-specific inductive biases. We show results on images, climate data, 3D shapes and scenes as well as audio and video, introducing VC-INR as the first INR-based method to outperform codecs as well-known and diverse as JPEG 2000, MP3 and AVC/HEVC on their respective modalities.

==> figures/concept_figure.tex <==
\begin{figure*}[t]
\begin{center}
\includegraphics[width=0.9\linewidth]{figures/concept_figure.pdf}
\end{center}
\caption{
An overview of the proposed \sname. We convert data points from diverse modalities into INRs where such INRs are compressed into a low-bit stream through neural compression.
}
\label{fig:concept}
\end{figure*}


==> section/acknowledgements.tex <==
We thank Hyunjik Kim and ‪Danilo J. Rezende for their insightful comments and feedback.
